The sharp constants in the real anisotropic Littlewood's $\boldsymbol{4 / 3}$ inequality and applications

The real anisotropic Littlewood's $4 / 3$ inequality is an extension of a famous result obtained in 1930 by J. E. Littlewood. It asserts that, for $a , b \in ( 0 , \infty )$, the following conditions are equivalent: $\bullet$ There is an optimal constant $\mathsf{L}_{ a , b }^{ \mathbb{R} } \in [ 1 , \infty )$ such that \[ \Biggl ( \, \sum_{ k = 1 }^{ \infty } \biggl ( \, \sum_{ j = 1 }^{ \infty } \bigl \lvert A \bigl ( \boldsymbol{e}^{ (k) } , \boldsymbol{e}^{ (j) } \bigr ) \bigr \rvert^a \biggr )^{ \frac{b}{a} } \Biggr )^{ \frac{1}{b} } \leq \mathsf{L}_{ a , b }^{ \mathbb{R} } \cdot \lVert A \rVert \] for every continuous bilinear form $A \colon c_0 \times c_0 \to \mathbb{R}$. $\bullet$ The values $a , b$ satisfy $a , b \geq 1$ and $\frac{1}{a} + \frac{1}{b} \leq \frac{3}{2}$. Several authors have obtained the values of $\mathsf{L}_{ a , b }^{ \mathbb{R} }$ for diverse pairs $( a , b )$. In this paper we provide the complete list of such optimal values, as well as new estimates for $\mathsf{L}_{ a , b }^{ \mathbb{C} }$ (the analog for continuous $\mathbb{C}$-bilinear forms), which are exact in several cases. As an application we prove, in terms of the values $\mathsf{L}_{ 1 , r }^{ \mathbb{C} }$, a variant of Khinchin's inequality for Steinhaus variables, and we provide estimates for the optimal $( q , s )$-cotype constants of the spaces $\ell_1 ( \mathbb{K} )$ (with $\mathbb{K} = \mathbb{R}$ or $\mathbb{C}$) in terms of the values $\mathsf{L}_{ 1 , q }^{ \mathbb{R} }$.

==> hksqrt.tex <==
% root symbol with hook
\usepackage{letltxmacro}
\LetLtxMacro{\OldSqrt}{\sqrt}
\newcommand{\ClosedSqrt}[1][\hphantom{3}]{\def\DHLindex{#1}\mathpalette\DHLhksqrt}
\makeatletter
    \newcommand*\bold@name{bold}
    \def\DHLhksqrt#1#2{%
        \setbox0=\hbox{$#1\OldSqrt{#2\kern 0.08em}$}\dimen0=\ht0\relax%
        \advance\dimen0-0.246\dimen0\relax% size of the added box is still 0.246 times ht0
        \setbox2=\hbox{\vrule height 1.346\dimen0 depth -\dimen0 width\ifx\math@version\bold@name1pt\else0.75pt\fi}%
        {\hbox{$#1\expandafter\OldSqrt\expandafter[\DHLindex]{#2\kern 0.08em}$}
        %\lower\ifx\math@version\bold@name0.242ex\else0.176ex\fi\box2
        \lower\ifx\math@version\bold@name0.135\dimen0\else0.103\dimen0\fi\box2
        }
    }
    % root index positioning and added space at the end, mostly noticeable in inline math mode
    \renewcommand*{\sqrt}[2][\ ]{\ClosedSqrt[\leftroot{0}\uproot{1}#1]{#2}\kern0.1em} 
\makeatother
